Opinion-Guided Reinforcement Learning

Human guidance is often desired in reinforcement learning to improve the performance of the learning agent. However, human insights are often mere opinions and educated guesses rather than well-formulated arguments. While opinions are subject to uncertainty, e.g., due to partial informedness or ignorance about a problem, they also emerge earlier than hard evidence can be produced. Thus, guiding reinforcement learning agents by way of opinions offers the potential for more performant learning processes, but comes with the challenge of modeling and managing opinions in a formal way. In this article, we present a method to guide reinforcement learning agents through opinions. To this end, we provide an end-to-end method to model and manage advisors' opinions. To assess the utility of the approach, we evaluate it with synthetic (oracle) and human advisors, at different levels of uncertainty, and under multiple advice strategies. Our results indicate that opinions, even if uncertain, improve the performance of reinforcement learning agents, resulting in higher rewards, more efficient exploration, and a better reinforced policy. Although we demonstrate our approach through a two-dimensional topological running example, our approach is applicable to complex problems with higher dimensions as well.

==> sections/old-text-snippets/approach.tex <==

\iffalse
\id{$\downarrow\downarrow\downarrow$ Moved these here$\downarrow\downarrow\downarrow$}

\todo{The set of hints forms a matrix $H  = S \times A$;}

\paragraph{Transformation of opinions to probabilities}
\todo{May want to normalize the values $p_i$ within each row to ensure that $0 \le p \le 1$ and $\sum p_i = 1$}
\begin{itemize}
    \item $\theta_{\text{prob2}}$ is an $m \times n$ matrix of probabilities $p$, such that $0 \le p \le 1$
\end{itemize}

\paragraph{Transformation of probabilities to opinions}
\begin{itemize}
    \item $\theta_{\text{opinion}}$ is an $m \times n$ matrix of binomial opinions such that 
$$\sum_{i=1}^m \sum_{j=1}^n \theta_{\text{opinion}}[i, j] = (b, d, u, a)$$
\end{itemize}

\paragraph{Converting probabilities to binomial opinions}
\begin{enumerate}
\item Set each element of $\theta_{\text{opinion}}$ 
$$\sum_{i=1}^m \sum_{j=1}^n \theta_{\text{opinion}}[i, j] = (p , 1-p , 0, p )$$
where 
$$p = \theta_{\text{prob1}}[i, j]$$


\end{enumerate}

\paragraph{Converting from fused opinions to probabilities}
$$\sum_{i=1}^m \sum_{j=1}^n[\theta_{\text{prob2}}] = b + a * u$$
where
$$b = [\iota[i, j]][0]$$
$$u = [\iota[i, j]][2]$$
$$a = [\iota[i, j]][3]$$


\subsubsection{Initializing $H$}

\todo{we should move these parts to a pseudo-algorithm}

\begin{enumerate}
    \item Set each element of $H$ to the neutral element (vacuous opinion in \cite{burgueno2023dealing}) $n = (0, 0, 1, 1/|A|)$ %such that $$\sum_{i=1}^m \sum_{j=1}^n \kappa[i, j] = (0, 0, 1, 1/n)$$
\end{enumerate}

\subsubsection{Inserting hints into $H$}
\begin{enumerate}
    \item Given an opinion $(s, a, (b, d, u, a))$, insert the hint $(b, d, u, a)$ at $\kappa[s, a]$ such that 
$$\kappa[s, a] = (b, d, u, a)$$
\end{enumerate}

\subsection{Transformation of numerical preferences to probabilities}
\textbf{Note:} See link for definition of soft-max\\
\url{https://pytorch.org/docs/stable/generated/torch.nn.Softmax.html}
\begin{itemize}
    \item \textbf{Numerical preferences} are expressed by the agent of the reinforcement algorithm as an $m \times n$ matrix $\theta$ of real numbers
    \item $\theta_{\text{prob1}}$ is an $m \times n$ matrix of probabilities $p$, such that $0 \le p \le 1$
\end{itemize}

\subsubsection{Converting from numerical preferences to probabilities}
\begin{enumerate}
    \item Compute the soft-max of $\theta$ and store in $\theta_{\text{prob}1}$ such that 
$$\theta_{\text{prob}1} = \text{soft-max}(\theta)$$

\end{enumerate}

\subsection{Transformations of probabilities to numerical preferences}
\textbf{Note: }See link for definition of inverse soft-max\\ \url{https://search.r-project.org/CRAN/refmans/ohenery/html/inv_smax.html}
\subsubsection{Converting from probabilities to numerical preferences} 
\begin{enumerate}
    \item Compute the inverse soft-max of $\iota$ and store in $\theta$ such that 
$$\theta = \text{soft-max}^{-1}(\iota)$$
\end{enumerate}

\fi


==> sections/old-text-snippets/discussion.tex <==
\subsection{Operationalization of the approach}

\todo{describe the typical lifecycle (see our models submission and Robbert's models paper from 2023) -- when to provide advice, by whom, etc} 


\begin{itemize}
    \item we used one-time advice prior to exploration, but there are other ways too
    \item advise during exploration
    \begin{itemize}
        \item pull-push
    \end{itemize}
\end{itemize}



\begin{itemize}
    \item Sequential has a better reinforced policy (heatmap b \& d have more dark cells than c \& e)
    \begin{itemize}
        \item Again, likely due to advisors at critical areas of map (start, goal, along path)
        \item As per above, advisor at start means agent navigates beginning of map better, can take more steps in early episodes and spend more time reinforcing the policy
    \end{itemize}
    \item Parallel has better exploration (heatmap c \& e have more cells explored than b \& d)
    \begin{itemize}
        \item The agent likely has to explore more in parallel mode because it does not get significant advice around the start or goal. The agent essentially has to explore in order to use the advice given in parallel mode because these cells are farther from start, goal, and path. 
        \item We need to note that sequential coop (particularly the advisor at the start) has more positive advice (+1) than parallel coop. This means sequential is not only telling agent what to avoid, but where to go, restricting its policy. 
            \item Hard to say if more exploration is due solely to advisor location
        \item Note that in parallel 10, agent explores top right of map more than parallel 5 even though in parallel 10, the advisor uses more negative advice in that area - Why is this happening? 
    \end{itemize}
\end{itemize}


\begin{itemize}
    \item sequential coop -- siloed environments
    \item parallel coop -- subject-matter expertise
\end{itemize}


\begin{itemize}
    \item Coop: in an A-C setup, the human can be considered the critic and the agent the actor. \todo{for our MPM4CPS paper: A-C-C architecture where the human is the top level C, RL is the middle C, and DSE is the A?}
\end{itemize}


%Suppose the agent had access to an oracle that could provide hints to the agent before beginning the task. The oracle’s hint may describe a path to the goal (a path based hint) or the hint may describe one or more tiles the agent should try to visit (state based hint). As the oracle’s hints describe information the agent would likely learn across many attempts, it is likely that with this information, the agent will learn the optimal path in fewer trials than without. However, the oracle’s hints come with a level of uncertainty about certain it is in the information it is providing. The agent must meaningfully use these hints and weigh the certainty of the oracle in future decision making.

%This example further extends into other reinforcement learning problems. In general, the agent is analogous to any decision making agent, and the oracle analogous to a human with some information about the task. The human can give the agent path based hints, or state based hints, with accompanying measures of belief about the hints.  This should help the agent reach an optimal solution with fewer trials and in less time that without human hints, as these hints give the agent information it would have had to find out on its own. \id{some of this explanation might go to either the background (most likely) or perhaps the approach.}


We foresee our approach to be adopted with a high utility primarily in situations with a scarce reward structure, where human creativity plays an important role. Such situations are, for example, problems with infeasible, inaccessible, hazardous, or costly states which, consequently, cannot be efficiently explored by the RL agent.


\begin{itemize}
    \item In order to gradually learn the optimal path to the goal, the agent needs to map the environment extensively. This might not always be feasible... \todo{hazardous, too expensive, unreachable, etc}

	\item analogy of guidance: subject-matter expertise (explain non-topology --- MODELS paper)
 
	\item what is a oracle good for? (A-C architectures, domain-specific orcales, etc)
	\item \todo{more content here to balance subsecs}
\end{itemize}

==> sections/old-text-snippets/uncertainty-in-rl.tex <==
%\kd{some notes to consider for the journal paper, just wasn't sure how to use them at the moment}
%    \begin{itemize}
%        \item perhaps more from \citet{hullermeier2021aleatoric} & \citep{guo2024survey}
%        \item \citet{neider2021advice} -- ``\textit{While assuming full knowledge of the reward machine is rightly deemed overly optimistic (see above), we believe that assuming no knowledge is overly pessimistic. Indeed, a typical situation will be between the two extremes: a human engineer certainly has some high-level knowledge about the reward function/machine and can often provide some sort of ``advice''.}''
%        \item \citet{scherf2022learning} -- Learning from Unreliable Human Action Advice
%       \begin{itemize}
%            \item concerned with \textit{consistency}, and not quantifying certainty
%        \end{itemize}
%        \item \citet{dasilva2020uncertainty} has agent request guidance when epistemic uncertainty is high and advising is available. They calculate uncertainty so maybe mention in uncertainty section as well?
%        \item \citet{cederborg2015policy} read more on this paper, has interesting notion of probability of teacher's evaluation being useful, similar to our use of $u$
%    \end{itemize}

%\subsubsection{Other -- Secondary studies}
%\begin{itemize}
%    \item \citet{lin2020review} -- review article. might be good to classify our approach.
%\end{itemize}
%


\subsection{Uncertainty in reinforcement learning}
A key feature of Machine Learning (ML) and Reinforcement Learning (RL) models is uncertainty. Models usually capture, predict, and reason about complex processes that are inherently uncertain.  Thus, these models require robust uncertainty modeling and quantification techniques in order to perform well in novel situations, as well as to ensure safe, efficient, and useful behavior. In terms of RL and ML models, uncertainty is generally classified as either aleatoric, or epistemic. Aleatoric uncertainty is the irreducible uncertainty due to the randomness or variability of a process. On the other hand, epistemic uncertainty is the reducible uncertainty that stems from a lack of information, or ignorance on the part of the observer \citep{hullermeier2021aleatoric}. 

In RL in particular, aleatoric uncertainty may be present in rewards, actions, and observations that are stochastic ~\citep{lockwood2022review}. This is dependent on the environment and will vary from case to case. Epistemic uncertainty in RL is present in regions of the state space that are unexplored or visited infrequently. This leads to the RL model over or underestimating policy or value functions. \citet{lockwood2022review} write an overview of several approaches used to quantify uncertainty in Deep Reinforcement Learning (DRL). 

Many works use a combination of statistical methods to estimate uncertainty, such as in \citet{kahn2017uncertainty}, where an RL framework that uses a neural network to estimate collision probabilities uses both bootstrapping and Monte-Carlo dropout to obtain accurate uncertainty measurements. Similarly, \citet{lutjens2019safe} present an RL framework for collision avoidance under uncertainty using bootstrapping and MC-dropout. In a method similar to bootstrapping, \citet{clements2019estimating} quantify epistemic and aleatoric uncertainty by learning the probability distribution of the value function using quantile parameterization as per \citet{dabney2018distributional}. \citet{charpentier2022disentangling} define desired behaviors that they expect the RL model to execute during training and testing under different types of uncertainty, and then use four uncertainty estimation methods that each capture uncertainty. These include MC Dropout, Ensemble, Deep Kernel Learning, and Evidential Networks. These works aim to capture uncertainty in order to improve an RL model's accuracy and performance, and do not aim to directly change epistemic uncertainty in the model. In contrast, count based methods, such as in \citet{bellemare2016unifying}, maintain a count of the number of times an agent has encountered each state, and biases the policy to choose actions that explore states with low counts in order to lower epistemic uncertainty. Our work aims to decrease the epistemic uncertainty by guiding the RL agent via opinions. These opinions increase the information available to the agent, and thus decreasing its epistemic uncertainty. 






